Unsupervised Learning of 3D Structure from Images

A key goal of computer vision is to recover the underlying 3D structure from 2D observations of the world. In this paper we learn strong deep generative models of 3D structures, and recover these structures from 3D and 2D images via probabilistic inference. We demonstrate high-quality samples and report log-likelihoods on several datasets, including ShapeNet [2], and establish the first benchmarks in the literature. We also show how these models and their inference networks can be trained end-to-end from 2D images. This demonstrates for the first time the feasibility of learning to infer 3D representations of the world in a purely unsupervised manner.

==> relatedWork.tex <==
%!TEX root = main.tex
\vspace{-2mm}
\section{Related Work}

Volumetric representations have been explored extensively for the tasks of object classification \cite{su2015multi, nair20093d, 
socher2012convolutional, wu20153d}, object reconstruction from images \cite{choy20163d}, volumetric denoising \cite{wu20153d, choy20163d} and density estimation \cite{wu20153d}. The model we present in this paper extends ideas from the current state-of-the art in deep generative modeling of images \cite{gregor2015draw,gregor2016compression,rezende2016one} to volumetric data. Since these models operate on smooth internal representations, they can be combined with continuous projection operators more easily than prior work.

On the other hand, mesh representations allow for a more compact, yet still rich, representation space. When combined with OpenGL, we can exploit these representations to more accurately capture the physics of the rendering process. Related work include deformable-parts models \cite{chaudhuri2011probabilistic, funkhouser2004modeling, 
kalogerakis2012probabilistic} and approaches from inverse graphics \cite{wu2015galileo,kulkarni2015picture,eslami2016attend,loper2014opendr}. 

Learning models of 3D structures directly from pixels has been a long-standing open problem. A number of approaches with different levels of underlying assumptions and feature engineering have been proposed in the literature. Traditional approaches to vision as inverse graphics \cite{mansinghka2013approximate, kulkarni2014inverse, loper2014opendr} and analysis-by-synthesis \cite{pero2012bayesian, wingate2011nonstandard, kulkarni2014deep, wu2015galileo} rely on heavily engineered visual features with which inference of object properties such as shape and pose is substantially simplified. More recent work in this domain \cite{kulkarni2014deep, dosovitskiy2015learning, choy20163d, 2016arXiv160503557Z} addresses some of these limitations by learning parts of the encoding-decoding pipeline depicted in figure \ref{fig:diagrams} in separate stages. To the best of our knowledge our results constitute the first demonstration of learning to model 3D representations end-to-end and directly from 2D images in an unsupervised manner. Further related work is discussed in appendix \ref{ap:relatedwork}.
